Where Graph Topology Matters: The Robust Subgraph Problem

Robustness is a critical measure of the resilience of large networked systems, such as transportation and communication networks. Most prior works focus on the global robustness of a given graph at large, e.g., by measuring its overall vulnerability to external attacks or random failures. In this paper, we turn attention to local robustness and pose a novel problem in the lines of subgraph mining: given a large graph, how can we find its most robust local subgraph (RLS)? We define a robust subgraph as a subset of nodes with high communicability among them, and formulate the RLS-PROBLEM of finding a subgraph of given size with maximum robustness in the host graph. Our formulation is related to the recently proposed general framework for the densest subgraph problem, however differs from it substantially in that besides the number of edges in the subgraph, robustness also concerns with the placement of edges, i.e., the subgraph topology. We show that the RLS-PROBLEM is NP-hard and propose two heuristic algorithms based on top-down and bottom-up search strategies. Further, we present modifications of our algorithms to handle three practical variants of the RLS-PROBLEM. Experiments on synthetic and real-world graphs demonstrate that we find subgraphs with larger robustness than the densest subgraphs even at lower densities, suggesting that the existing approaches are not suitable for the new problem setting.

==> dfn.tex <==
% shorthands for naming conventions
\newcommand{\question}[1]{{\emph{#1}}}
\newcommand{\ksa}{K\_softAND}
\newcommand{\myK}{k}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\goal}[1]{ {\noindent {$\Rightarrow$} \em {#1} } }
\newcommand{\hide}[1]{}
\newcommand{\comment}[1]{ {\footnotesize {#1} } }
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proof}{Proof}
\newtheorem{defn}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{observation}{Observation}
% macro symbol definitions
\newcommand{\reminder}[1]{{\bf *** #1 ***}}
\newcommand{\prop}{{\em{CEPS}}}       % name for the proposed method
\newcommand{\propfull}{{{center-piece}}}       % full name for the proposed method
\newcommand{\pmetric}{\emph{meeting probability}}%name for the proposed goodness score
\newcommand{\ssp}{\emph{steady-state probability}}%name for steady-state probability
\newcommand{\extract}{\emph{EXTRACT}}%name for the extract algorithm
\newcommand{\lqu}{``}%left double quatation
\newcommand{\rqu}{''}%right double quatation
%\newcommand{\modul1}{\tt{IndividualScoreCalculation}}       % name for the Individual Score Calculation
%\newcommand{\modul2}{\tt{Combination}}       % name for the combination
%\newcommand{\modul3}{\tt{EXTRACT}}       % name for the dynamic programming
\newcommand{\qi}{q_i}  %index for a single query node i
\newcommand{\pd}{pd}  %promising node
\newcommand{\QN}{{Q}}       % count of query nodes
\newcommand{\Qset}{{\cal Q}}    % set of query nodes
\newcommand{\Qsetm}{{\cal \acute{Q}}}    % set of query nodes, not including the last query node
\newcommand{\Qsetzero}{{\cal \varnothing}}    % null set of query nodes, not including the last query node
\newcommand{\collision}{r}  % so that we can change it, to say,
                %        r-endezvous, or m-eeting
\newcommand{\cij}{ \collision_{i,j}}    % collision probability
\newcommand{\cijpar}{ \collision{(i,j)}} % collision probability, also
\newcommand{\cqj}{ \collision ( \Qset, j)} % group collision probability
\newcommand{\cqjK}{ \collision ( \Qset, j, \myK)} % group collision probability
\newcommand{\cqjQ}{ \collision ( \Qset, j, \QN)} % group collision probability for AND query
\newcommand{\cqjone}{ \collision ( \Qset, j, 1)} % group collision probability for OR query
\newcommand{\cqHK}{ \collision ( \Qset, \Hgraph, \myK)} % score for matrix H, for k-and query
\newcommand{\Hgraph}{ { \cal H}} % the connection subgraph
\newcommand{\mat}[1]{{\bf #1}}   % matrix: bold
\newcommand{\matC}{ \mat{R}} % the collision/rendezvous matrix
\newcommand{\matW}{ \mat{W}} % the weight matrix
\newcommand{\matP}{ \mat{P}} % the transition matrix
\newcommand{\matS}{ \mat{S}} % the graph Laplacian
\newcommand{\matD}{ \mat{D}} % the degree matrix
\newcommand{\matQ}{ \mat{Q}} % the system matrix
\newcommand{\matWnorm}{ \tilde{\mat{W}}} % the weight matrix
\newcommand{\matWnorma}{\tilde{{\mat{W}}}_{1}} % within partition matrix;
\newcommand{\matWnormai}{\tilde{{\mat{W}}}_{1,i}} % within partition matrix;
\newcommand{\matWnormb}{\tilde{{\mat{W}}}_{2}} % cross partition matrix;
\newcommand{\myB}{\mat{U}} % node-concept matrix;
\newcommand{\myC}{\mat{S}} % concept-concept matrix;
\newcommand{\myD}{\mat{V}} % concept-node matrix;
\newcommand{\FastRWR}{B\_LIN} % Abbreveate for proposed method;
\newcommand{\SimFastRWR}{NB\_LIN} % Abbreveate for simplified proposed method;
\newcommand{\FastBitRWR}{bNB\_LIN} % Abbreveate for simplified proposed method for bipartite;

%abbr. for the dataset
\newcommand{\CorelFive}{Co5000} % Abbreveate for Corel 5000 image Dataset
\newcommand{\CorelMMG}{CoMMG} % Abbreveate for Corel 52,000 image Dataset for cross-media correlation discovery
\newcommand{\DblpAp}{AP} % Abbreveate for DBLP Author-paper Dataset
\newcommand{\DblpAc}{AC} % Abbreveate for DBLP Author-conference Dataset

\newcommand{\edge}{ {(j,l)}}    % an edge
\newcommand{\cqedge}{ \collision ( \Qset, \edge)} % score for matrix H, for k-and query
\newcommand{\cqedgeK}{ \collision ( \Qset, \edge, \myK)} % score for matrix H, for k-and query
\newcommand{\ciedge}{ \collision ( i, \edge)} % score for matrix H, for k-and query

\newcommand{\unitvi}{ \vec{e}_i} % unit vector, with all zeros except at i






\newcommand{\GPL}{{Densification Power Law}}

\newcommand{\GPLplot}{{DPL plot}}
\newcommand{\CCDC}{{Difficulty Constant}}
\newcommand{\CCDF}{{Difficulty Function}}
\newcommand{\CGA}{Community Guided Attachment}
\newcommand{\DCGA}{Dynamic Community Guided Attachment}
\newcommand{\gdiff}{Scale-free Difficulty}
\newcommand{\ssda}{Scale-free Difficulty Assumption}

% dataset shorthands:
\newcommand{\arxiv}{{arXiv}}
\newcommand{\patents}{{\tt Patents}}
\newcommand{\authorpaper}{{\tt AuthorPaper}}
\newcommand{\autonsys}{{\tt AS}}

\newcommand{\dbar}{\bar{d}}
\newcommand{\Alpha}{\alpha}
\newcommand{\Beta}{\beta}

